North Polar Spur/Loop I: gigantic outskirt of the Northern Fermi bubble or nearby hot gas cavity blown by supernovae?

Radio continuum, microwave and gamma-ray images of the Milky Way reveal a conspicuous, loop-like structure that fills almost half of the northern Galactic hemisphere, called Loop I. The interior of Loop I is shining in soft X-rays, and its eastern base is a bright, elongated structure dubbed the North Polar Spur (NPS). After 40 years of debates, two contradictory views of Loop I/NPS are still defended: on the one hand, the NPS is a volume of expanding hot gas that envelops and extends the northern Fermi Bubble (FB) known to be blown by the Galactic center, and Loop I marks the shock front; on the other hand, the NPS is a nearby cavity of hot gas blown by supernovae, Loop I is its shock front and they are coincidentally located in the direction of the FB. To an observer at the Sun, both structures can produce the same perspective view, although the former has a size comparable to the Milky Way itself, and the latter a diameter of a few hundreds parsecs. The energy involved varies by 3-4~orders of magnitude, and the solution has various important consequences. I discuss recent results which have a connection with Loop I/NPS, overlooked or used as arguments in the two opposite ways. They involve very different spacecraft, from a 12 Kg Cubesat (HaloSat) to major space-borne observatories (HST, Gaia, and Spektr-RG). I make use of 3D~maps of dust and a massive star catalog. Considering all constraints, it is clear that there is no entirely local or entirely distant scenario that is free from contradictions with some of the data analyses or from improbable coincidences. I discuss a speculative scenario, partially inspired by recent BF and Milky Way gas models, combining near and far aspects and seeming to be able to meet the various constraints. However, new data and models are needed to bring the controversy to a close and we can still expect new episodes of this long story.

==> CR-1col.tex <==
%% CR parameters for 1 col. series
\textwidth=140truemm
\oddsidemargin.6mm
\evensidemargin.6mm
\columnsep=18pt \columnseprule=0pt
\skip\footins=18pt plus12pt
\skip\@mpfootins=\skip\footins
\abstractmargin2em
\abstractmarginL\abstractmargin
\abstractmarginR\abstractmargin
%% parameters C&J
\pretolerance=600
\tolerance=2400 % INITEX sets this to 10000
\hbadness=2500
\vbadness=1000
\linepenalty=10
\hyphenpenalty=40
\exhyphenpenalty=50
\binoppenalty=700
\relpenalty=500
\clubpenalty=3000
\widowpenalty=4000 
\displaywidowpenalty=6000
\brokenpenalty=3000
\predisplaypenalty=10000
\doublehyphendemerits=600
\finalhyphendemerits=4000
\adjdemerits=10000
\emergencystretch=1.5em
\uchyph=1
\hfuzz.5pt
\lineskip=0pt 
\endinput


==> CR-gen.tex <==
%% 2019-03-25, second+epsilon alpha version 
%% CR style file, all series
%% Metadata
%  Journal title
\protected@edef\currentjournaltitle{Comptes Rendus. \CDRcrasseries}
%  journal publisher
\protected@edef\currentjournalpublisher{Acad\'emie des sciences, Paris}
%
\definecolor{AcademyGreen}{rgb}{0,0.6,.4}
%% The website
\xdef\journalURL{https://comptes-rendus.academie-sciences.fr/\cdr@journaldirectory/}%
%
  \let\cdr@shortresps\@empty
  \let\cdr@resps\@empty
  \let\cdr@specialtitle@french\@empty
  \let\cdr@specialtitle@english\@empty
  \let\cdr@specialabstract@french\@empty
  \let\cdr@specialabstract@english\@empty
\let\cdr@presentedby\@empty
\def\PresentedBy#1{\gdef\cdr@presentedby{#1}}
\def\@set@presentedby{\cdr@presentedby@name\cdr@presentedby\@addpunct.}
\if@francais
\def\cdr@presentedby@name{Pr\'esent\'e par }
\else
\def\cdr@presentedby@name{Presented by }
\fi
%
\def\TopicFR#1{\gdef\cdr@topicFR{#1}}
\def\TopicEN#1{\gdef\cdr@topicEN{#1}}
\def\TopicEF#1#2{\gdef\cdr@topicEN{#1}\gdef\cdr@topicFR{#2}}
\def\RubricFR#1{\gdef\cdr@rubricFR{#1}}
\def\RubricEN#1{\gdef\cdr@rubricEN{#1}}
\def\RubricEF#1#2{\gdef\cdr@rubricEN{#1}\gdef\cdr@rubricFR{#2}}
%
%%geometry
\paperwidth=192truemm
\paperheight=262truemm
\ifx\undefined\pdfpagewidth\else
\pdfpagewidth\paperwidth
\pdfpageheight\paperheight
\fi
\setlength{\topmargin}{-12truemm}%
\setlength{\topskip}{13pt}
\setlength{\baselineskip}{12.2pt}
\setlength{\textheight}{\topskip}
\addtolength{\textheight}{48\baselineskip}%
%\textheight=210truemm
\headheight=10pt
\headsep 10mm
\marginparsep=10pt
\marginparpush=5pt
\marginparwidth=20mm
\footskip 14mm 

\pretolerance=600
\tolerance=2400 % INITEX sets this to 10000
\hbadness=2500
\vbadness=1000
\linepenalty=10
\hyphenpenalty=40
\exhyphenpenalty=50
\binoppenalty=700
\relpenalty=500
\clubpenalty=3000
\widowpenalty=4000 
\displaywidowpenalty=6000
\brokenpenalty=3000
\predisplaypenalty=10000
\doublehyphendemerits=600
\finalhyphendemerits=4000
\adjdemerits=10000
\emergencystretch=1.5em
\uchyph=1
\hfuzz.5pt
\lineskip=0pt 

%% 
\normalparindent=12pt
\parindent=\normalparindent
\frenchspacing
%% ajust 10 pt interligne Fourier
\def\@mainsize{10}\def\@ptsize{0}%
  \def\@typesizes{%
    \or{5}{6}\or{6}{7}\or{7}{8}\or{8}{10.1}\or{9}{11.2}%
    \or{10}{12.2}% normalsize
    \or{\@xipt}{13}\or{\@xiipt}{14}\or{\@xivpt}{17}%
    \or{\@xviipt}{20}\or{\@xxpt}{24}}%
  \normalsize \linespacing=\baselineskip
%
%
\let\@listI\@listi
\@listi
%
%% Fonts
\ifcdr@m@nuscript
\IfFileExists{fourier.sty}{%
\PackageWarning{Mersenne/comptes Rendus}{Fourier font used}  
\usepackage{fourier}}
{\PackageWarning{Mersenne/comptes Rendus}{Fourier font not installed,
    the article will have to be retypeset!}}  
\else
\usepackage[expert]{fourier}
\pdfmapfile{=fourier.map}
\pdfmapfile{=fourier-utopia-expert.map}
\fi
\AtBeginDocument{\ifx\textsb\undefined\let\textsb\textbf\fi}
\def\@captionheadfont{\bfseries}%
\def\cdr@up{}%
%% Float captions
\captionindent=\normalparindent
\long\def\@makecaption#1#2{%
  \setbox\@tempboxa\vbox{\color@setgroup
    \advance\hsize-2\captionindent\noindent
    \@captionfont\@captionheadfont#1%
    \def\cdr@tmp@{\ignorespaces \ifHy@nesting \hyper@@anchor {\@currentHref }{}\else
      \Hy@raisedlink {\hyper@@anchor {\@currentHref }{\relax }}\fi}%
    \def\cdr@tmp@@{#2}%
%    \@xp\ifx\csname hyper@@anchor\endcsname\relax
    \ifx\cdr@tmp@@\cdr@tmp@\cdr@tmp@\else
    \def\cdr@tmp@{\ignorespaces}%
    \ifx\cdr@tmp@@\cdr@tmp@\else% \@xp\@ifnotempty\@xp{\@cdr#2\@nil}{
    \captionseparator\@captionfont\cdr@up\enspace#2
    \fi\fi
    \unskip\kern-2\captionindent\par
    \global\setbox\@ne\lastbox\color@endgroup}%
  \ifhbox\@ne % the normal case
    \setbox\@ne\hbox{\unhbox\@ne\unskip\unskip\unpenalty\unkern}%
  \fi
  % \ifdim\wd\@tempboxa=\z@ % this means caption will fit on one line
  %   \setbox\@ne\hbox to\columnwidth{\hss\kern-2\captionindent\box\@ne\hss}%
  % \else % tempboxa contained more than one line
    \setbox\@ne\vbox{\unvbox\@tempboxa\parskip\z@skip
        \noindent\unhbox\@ne\advance\hsize-2\captionindent\par}%
%  \fi
  \ifnum\@tempcnta<64 % if the float IS a figure...
    \addvspace\abovecaptionskip
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
  \else % if the float IS NOT a figure...
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
    \nobreak
    \vskip\belowcaptionskip
  \fi
\relax
}
%% unnumbered/unnamed captions
\def\silentcaption{%
   \ifx\@captype\@undefined
     \@latex@error{\noexpand\caption outside float}\@ehd
     \expandafter\@gobble
   \else
%     \refstepcounter\@captype
     \expandafter\@firstofone
   \fi
   {\@dblarg{\S@caption\@captype}}%
}
\long\def\S@caption#1[#2]#3{%
  \par
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
    {\protect\numberline{\ }{\ignorespaces #2}}%
  \begingroup
    \@parboxrestore
    \if@minipage
      \@setminipage
    \fi
    \normalsize
    \S@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}
\long\def\S@makecaption#1#2{%
  \setbox\@tempboxa\vbox{\color@setgroup
    \advance\hsize-2\captionindent\noindent
%    \@captionfont\@captionheadfont#1%
    \def\cdr@tmp@{\ignorespaces \ifHy@nesting \hyper@@anchor {\@currentHref }{}\else
      \Hy@raisedlink {\hyper@@anchor {\@currentHref }{\relax }}\fi}%
    \def\cdr@tmp@@{#2}%
%    \@xp\ifx\csname hyper@@anchor\endcsname\relax
    \ifx\cdr@tmp@@\cdr@tmp@\cdr@tmp@\else
    \def\cdr@tmp@{\ignorespaces}%
    \ifx\cdr@tmp@@\cdr@tmp@\else% \@xp\@ifnotempty\@xp{\@cdr#2\@nil}{
%    \captionseparator\@captionfont\cdr@up\enspace
#2
    \fi\fi
    \unskip\kern-2\captionindent\par
    \global\setbox\@ne\lastbox\color@endgroup}%
  \ifhbox\@ne % the normal case
    \setbox\@ne\hbox{\unhbox\@ne\unskip\unskip\unpenalty\unkern}%
  \fi
  % \ifdim\wd\@tempboxa=\z@ % this means caption will fit on one line
  %   \setbox\@ne\hbox to\columnwidth{\hss\kern-2\captionindent\box\@ne\hss}%
  % \else % tempboxa contained more than one line
    \setbox\@ne\vbox{\unvbox\@tempboxa\parskip\z@skip
        \noindent\unhbox\@ne\advance\hsize-2\captionindent\par}%
%  \fi
  \ifnum\@tempcnta<64 % if the float IS a figure...
    \addvspace\abovecaptionskip
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
  \else % if the float IS NOT a figure...
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
    \nobreak
    \vskip\belowcaptionskip
  \fi
\relax
}
% 
%% Page layout
\pagenumbering{arabic}%
%% 1st page
\def\ps@firstpage{\count@=\currentyear
  \ps@plain
  \def\@oddfoot{{\scriptsize    
      ISSN (electronic) : \@Eissn\hfill\texttt{\url{\journalURL}}
}}
  \let\@evenfoot\@oddfoot
  \def\@oddhead{\@serieslogo\hss}%
  \let\@evenhead\@oddhead % in case an article starts on a left-hand page
}
%
%% Identificiation article 1st page
\def\prepageinfo{p.\, }
\def\pageinfosep{-} 
\def\@logofont{\footnotesize} 
\def\article@logo{%
    \set@logo{%
        \hsize\textwidth
        {\Large\textit{Comptes Rendus\\ \CDRcrasseries}\\[2pt]}% 
        \ifcdr@m@nuscript%
            \textbf{Draft}
        \else
            \ifcdr@Attached
                Supplementary material to the article available at:
            \else
                \ifcdr@efirst
                    Online first%
                    \ifx\@dateposted\@empty\else, {\selectlanguage{english}\printdate{\@dateposted}}\fi
                    % \ifx\@empty\@dateposted\else
                    %     , posted online {\selectlanguage{english}\printdate{\@dateposted}}
                    % \fi
                \else
                    \textbf{\currentyear}, \currentvolume, \no\currentissue, \prepageinfo\pageinfo
                \fi	
            \fi
            \\\texttt{\printDOI}
        \fi
        \hfill\raisebox{-3mm}[0pt][0pt]{\includegraphics[height=16mm]{Logo_Academie_grisfonce.pdf}}%
        \ifcdr@Attached\else\\[18bp]\centerline{\rule{.8\textwidth}{1.5bp}}\fi
    }
}% end \article@logo
%
%%  Copyright
\def\@setcopyright{}%
%% Standard pages
\def\ps@headings{%
    \ps@empty
    \def\@evenhead{%
        \rlap{\thepage}{}%\scshape
        \footnotesize\def\lastname####1{{####1}}%
        \hfil
        \def\thanks{\protect\thanks@warning}%
        \TopAuthors{}{}\hfil
    }%
    \def\@oddhead{%
        \let\\\relax
        \hfil
        \def\thanks{\protect\thanks@warning}%
        {\footnotesize\TopAuthors{}{}}\hfil
        \llap{\thepage}{}%
    }%
    \let\@mkboth\cdr@markboth
    \def\@oddfoot{%
        \footnotesize
        \textit{\shortpublname} ---
        \ifcdr@m@nuscript
            Draft, \today
        \else
            \ifcdr@Attached
                Supplementary material
            \else
                \ifcdr@efirst
                    Online first%
                    \ifx\@dateposted\@empty\else, {\selectlanguage{english}\printdate{\@dateposted}}\fi
                \else
                    \textbf{\currentyear}, \currentvolume, \no\currentissue, \pageinfo
                \fi
            \fi
        \fi
        \hfil
    }%
    \let\@evenfoot\@oddfoot
}
%
\def\currentyear{0000}

%% Alternative code for title/editors of special volumes
%% To be evaluated later
% \ifcdr@volume
%  \def\maketitle{%\@makePDFinfo
%   \def\cdrsom@out@filename{\cdr@idvol.cdrsom}%
%   \@makeSOM
%  } 
%  \def\enddoc@text{}
% \else
%   \let\cdr@specialvolshortresps\@empty
%   \let\cdr@specialvolresps\@empty
%   \let\cdr@specialvoltitle@french\@empty
%   \let\cdr@specialvoltitle@english\@empty
%   \let\cdr@specialvolabstract@french\@empty
%   \let\cdr@specialvolabstract@english\@empty
% \AtBeginDocument{%
% \begingroup\makeatletter
% \newcommand\SomLine[9]{%
%   \gdef\cdr@specialvolshortresps{#1}%
%   \gdef\cdr@specialvolresps{#2}%
%   \gdef\cdr@specialvoltitle@french{#5}%
%   \gdef\cdr@specialvoltitle@english{#4}%
%   \gdef\cdr@specialvolabstract@french{#7}%
%   \gdef\cdr@specialvolabstract@english{#6}%
%   }%
% \InputIfFileExists{../\CDRidvol.cdrsom}{%
% \message{** Fichier  \CDRidvol.cdrsom charg\'e pour
%   cet article **^^J}}{%
% \message{** Pas de fichier \CDRidvol.cdrsom  pour ce volume !**^^J}}%
% \makeatother\endgroup}
% \fi

\pagestyle{headings}%
%
\setlength{\@titletopskip}{26\p@}
\setlength{\@titlebotskip}{0\p@}
%% title presentation 

\let\overtitlebyhand\relax

\def\CDRtitleSep{\,/\,}

\def\@settitle{%
    \begin{flushleft}
        \vspace*{10pt}

        \strut
        \ifx\TITREspecial\@empty\else % This is part of a thematic issue
            \Large
            \ifx\overtitlebyhand\relax
                \ifx\cdr@specialtitle@english\@empty
                    \MissingInfo{Thematic issue title missing!}
                \else
                    \ifcdr@swaptitles\@title\else\cdr@specialtitle@english\fi
                    \ifx\cdr@specialtitle@french\@empty\else
                        \CDRtitleSep{\itshape\ifcdr@swaptitles\@alttitle\else\cdr@specialtitle@french\fi}
                    \fi
                \fi
            \else
                \overtitlebyhand
            \fi
        \fi      

    \vspace*{4pt}
 
    \@setTopicORRubric

    \addvspace{10pt}

    \def\baselinestretch{1.2}\large

    {\Huge\ifcdr@swaptitles\cdr@specialtitle@english\else
        \ifcdr@Attached Supplementary material: \fi\@title
    \fi\par}

    {\huge\itshape
        \ifx\@alttitle\@empty\else   
            \vspace*{14pt}
            \ifcdr@swaptitles\cdr@specialtitle@french\else
                \ifcdr@Attached Document compl\'ementaire\,: \fi\@alttitle % TODO French spacing for lt title
            \fi
            \par
        \fi}
 
    \vspace*{16pt}

    \end{flushleft}%
}
%
\def\CDRtopicSep{\,/\,}%
\def\CDRrubricSep{\,/\,}%
\def\@setTopicORRubric{%
    \if@francais
        \ifx\cdr@topicFR\@empty % rubric and topic mutually exclusive
            \ifx\cdr@rubricFR\@empty\else
                {%\textbf
                    \large\cdr@rubricFR
                    \ifx\cdr@rubricEN\@empty\else\CDRrubricSep\itshape\cdr@rubricEN\fi
                }%
            \fi
        \else
            {%\textbf
                \large\cdr@topicFR
                \ifx\cdr@topicEN\@empty\else\CDRtopicSep\itshape\cdr@topicEN\fi
            }%
        \fi
    \else
        \ifx\cdr@topicEN\@empty % rubric and topic mutually exclusive
            \ifx\cdr@rubricEN\@empty\else
                {%\textbf
                    \large\cdr@rubricEN
                    \ifx\cdr@rubricFR\@empty\else\CDRrubricSep\itshape\cdr@rubricFR\fi
                }%
            \fi
        \else
            {%\textbf
                \large\cdr@topicEN
                \ifx\cdr@topicFR\@empty\else\CDRtopicSep\itshape\cdr@topicFR\fi
            }%
        \fi
    \fi
}

\let\@ESM\@empty
\newcommand\ESM[1]{\def\@ESM{#1}}

\def\cdr@preabstracthook{\par\bigskip}
\def\cdr@interabstracthook{\par}%\smallskip}
\def\cdr@postabstracthook{%
    \@@par\smallskip
    \ifx\@empty\@keywords\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setkeywords}\smallskip
    \fi
    \ifx\@empty\@altkeywords\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setaltkeywords}\smallskip
    \fi
    \ifx\@empty\@subjclass\else 
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setsubjclass}\smallskip
    \fi
    \ifx\@empty\thankses\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setthanks}\smallskip
    \fi
    \ifx\@empty\@ESM\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setESM}\smallskip
    \fi
    \@@par{\abstractfont\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setdate}\par}
    \bigskip\bigskip
}
%
\def\CDRextrafirstfootnotetext{}
\def\abstractheadfont{\bfseries}
\def\@setabstracthead{{\abstractheadfont\abstractname\unskip.\kern.25em\ignorespaces}}
\def\@setaltabstracthead{{\abstractheadfont\altabstractname\unskip.\kern.25em\ignorespaces}%
}
%
%% authors
\def\@firstauthor#1\and#2\stop{#1}
\def\shortrunauthors{\gdef\@maketitle@shortauthors@hook{\def\topauthors{\@xp\@firstauthor\authors\stop\ \etal}}}
\def\shortrunPDGauthors{\g@addto@macro\@maketitle@shortauthors@hook{\def\PDGauthors{\@xp\@firstauthor\authors\stop\ \etal}}}
 \if@francais
  \def\manuscriptname{Manuscrit}%
  \def\receivedname{re\c cu}%
  \def\revisedname{r\'evis\'e}%
  \def\acceptedname{accept\'e}%
  \def\@@and{et}%
 \else
  \def\manuscriptname{Manuscript}%
  \def\receivedname{received}%
  \def\revisedname{revised}%
  \def\acceptedname{accepted}%
  \def\@@and{and}%
 \fi
%
\AtBeginDocument{\ifx\@daterevised\@dateaccepted\global\cdr@revisedacceptedtrue\fi
\ifx\@datereceived\@dateaccepted\global\cdr@receivedacceptedtrue\fi}
%
%%%%% presentation auteurs 
%\def\@@and{\&}
 \def\author@andify{%
   \nxandlist {\unskip ,\penalty-2 \space\cdr@count@hasaddr=\z@\ignorespaces}%
     {\unskip {} \cdr@count@hasaddr=\z@\@@and~}%
     {\unskip {} \penalty-2  \cdr@count@hasaddr=\z@\@@and~}%
 }
% \def\@maketitle@shortauthors@hook{\msia@shortauthor@andify\shortauthors\let\topauthors\shortauthors}
\newcount\cdr@thankcount
\cdr@thankcount\z@
\ifcdr@LTXGrid\else
\def\@alph#1{\ifcase#1\or a\or b\or c\or d\else\@ialph{#1}\fi}
\def\@ialph#1{\ifcase#1\or \or \or \or \or e\or f\or g\or h\or i\or j\or
 k\or l\or m\or n\or o\or p\or q\or r\or s\or t\or u\or v\or w\or x\or
 y\or z\or aa\or bb\or cc\or dd\or ee\or ff\or gg\or hh\or ii\or jj\or
 kk\or ll\or mm\or nn\or oo\or pp\or qq\or rr\or ss\or tt\or uu\or
 vv\or ww\or xx\or yy\or zz\else\@ctrerr\fi}
\fi
\def\cdr@CorrespondingAuthorIs{0}
\def\CDRorcid#1{\relax}
\let\IsEqualContrib\relax
\newcount\ContrA\ContrA=\z@
\let\IsCorresp\relax
\newcount\CorrA\CorrA=\z@
\def\display@orcid#1{%
  \href{https://orcid.org/#1}{%
    \raisebox{.7ex}[0pt][0pt]{%
%      \includegraphics[height=1.1ex]{orcid.png}{}%
      \includegraphics[height=1.1ex]{orcid-bw.png}}%
%{\usefont{TU}{academicons}{m}{n}\symbol{"E9D9}}}%
    }
}
\newcount\cdr@count@hasaddr\cdr@count@hasaddr=\z@%
\def\@setauthors{%
  \begingroup
  \def\CDRorcid##1{\kern1pt\display@orcid{##1}}%
  \def\IsCorresp{\textsuperscript{$*$,}\global\advance\CorrA\@ne\relax}%
  \def\IsEqualContrib{\textsuperscript{$\#$,}\global\advance\ContrA\@ne\relax}%}%
  \def\thanks{\protect\thanks@warning}%
  \author@andify\authors
  \def\\{\space}%
  \def\Same{\same}%
  \def\New{\new}%
  \def\hasaddress##1##2{%
    \ifnum\cdr@count@hasaddr=\z@\kern.1em\fi
    \@ifempty{##1}{% cas pas sameaddress
%%�increment de compteur
\global\advance\cdr@thankcount\@ne%
\textsuperscript{\ifnum\cdr@count@hasaddr>\z@, \fi
  \textit{\@alph\cdr@thankcount}}%
}{% cas sameaddress
\def\What{##1}\ifx\What\Same
%%�pas d'increment de compteur
\textsuperscript{\ifnum\cdr@count@hasaddr>\z@, \fi
  \textit{\@alph\cdr@thankcount}}%
\else\ifx\What\New
%%�increment de compteur
\global\advance\cdr@thankcount\@ne%
\textsuperscript{\ifnum\cdr@count@hasaddr>\z@, \fi
  \textit{\@alph\cdr@thankcount}}%
\else
%% manual numbering mode, produced by addressSameAs
\count@=##1\relax
\textsuperscript{\ifnum\cdr@count@hasaddr>\z@, \fi
  \textit{\@alph\count@}}%
\fi\fi}\advance\cdr@count@hasaddr\@ne}%
%\begin{minipage}[t]{.9\linewidth}\raggedright
\begingroup\hsize=.9\linewidth\raggedright
\large\textsb{\authors}\hfill\break%
  \ifx\@empty\contribs \else \\\penalty-3 \space \@setcontribs
  \@closetoccontribs \fi
  \par
  \endgroup
%\end{minipage}
\endgroup
  \ifnum\CorrA=\z@\else{{\def\@thefnmark{\rule{0pt}{10pt}$*\,$}%
    \@footnotetext{\def\CDRss{\ifnum\CorrA>\@ne\relax s\fi}\if@francais
      Auteur\CDRss\ correspondant\CDRss\else Corresponding
      author\CDRss\fi. \CDRextrafirstfootnotetext}}}\fi
  \ifnum\ContrA=\z@\else{{\def\@thefnmark{\rule{0pt}{10pt}$\#\,$}%
    \@footnotetext{\if@francais
      Contributions \'egales\else Contributed equally\fi.}}}\fi
}%
\def\@setafterauthor{%
  \vglue3mm%
%  \hspace*{0pt}%
\begingroup\hsize=10cm\advance\hsize\abstractmarginL\raggedright
\noindent
%\hspace*{\abstractmarginL}\begin{minipage}[t]{10cm}
   \leftskip\abstractmarginL
  \normalfont\Small
  \@afterauthor\par
\endgroup
\vskip2pt plus 3pt minus 1pt
}
\def\@afterauthor{%
    \ifx\@empty\addresses\else
        \@setaddresses\par
        \ifcdr@GroupEmails
            \ifcdr@existcurraddr
                \@setcurraddr\par
            \fi
            \@setemails\par
        \fi
        \bigskip%
    \fi
    \ifx\postaddressinfo\relax\else\textbf{\postaddressinfo}\par\bigskip\fi
}
\newif\ifcdr@existcurraddr\cdr@existcurraddrfalse
\def\@setaddresses{%\par
  \begingroup
  \cdr@thankcount\z@
   \ifcdr@hyperref  \url@samestyle
   \else\def\url##1{##1}%
   \def\href##1##2{##2}\fi
   \def\affiliationonly##1{##1}%
   \def\snailmailonly##1{\relax}%
   \def\lastname##1{\relax}%
   \def\firstname##1{\relax}%
   \def\hasthanks##1{##1\@addpunct.\@par}%
   \def\hasaddress##1{\relax}%
   \def\doauthorinfo##1{\@@par\textit{##1}}%
   \def\author##1{%\ifnum\cdr@notes@adress=\z@\else\@@par\indent\fi\global\advance\cdr@notes@adress1
     % \textsuperscript{\@alph\cdr@notes@adress}\kern.2em
     \def\\{ \ignorespaces}\ignorespaces}%
   \def\address##1##2{\begingroup
   \@ifempty{##1}{% cas pas addressSameAs
     \ifnum\cdr@thankcount>\z@\par\vskip4pt\fi\global\advance\cdr@thankcount\@ne
     \textsuperscript{\textit{\@alph\cdr@thankcount}}\kern.2em{\ignorespaces##2\unskip}}{}\endgroup}%
   \def\curraddr##1##2{%% Showing emails authorwise? Let's assume this follows the same logic as emails grouping.
     \ifcdr@GroupEmails\global\cdr@existcurraddrtrue\else
     \begingroup
     \@ifnotempty{##2}{\@@par\curraddrname{}\textit{\thsp:} %
       {\ignorespaces##2\unskip}\endgroup}\fi}%
   \def\email##1##2{%% Showing emails authorwise?
     \ifcdr@GroupEmails\else
     \begingroup
     \@ifnotempty{##2}{\@@par\emailaddrname{}%
       \@ifnotempty{##1}{ (##1)}\textit{\thsp:} %
       \href{mailto:##2}{##2}}\endgroup\fi
   }%
   \def\urladdr##1##2{\begingroup
%     \def~{\char`\~}%
     \@ifnotempty{##2}{\@@par\urladdrname{}\textit{\thsp:} %
       \url{##2}}\endgroup}%
   \addresses%\@addpunct.%
   \endgroup
 }
\def\@setemails{%\par
  \begingroup
   \cdr@thankcount\z@
   \ifcdr@hyperref  \url@samestyle
   \else\def\url##1{##1}%
   \def\href##1##2{##2}\fi
   \def\affiliationonly##1{\relax}%
   \def\snailmailonly##1{\relax}%
   \def\lastname##1{\relax}%
   \def\firstname##1{\relax}%
   \def\hasthanks##1{\relax}
   \def\hasaddress##1{\relax}%
   \def\author##1{}%\ifnum\cdr@thankcount=\z@\else, \fi}
   \def\address##1##2{\relax}%
   \def\curraddr##1##2{\relax}%
   \def\doauthorinfo##1{\relax}%
   \def\email##1##2{%% Showing emails authorwise?
     \ifcdr@GroupEmails
     \begingroup
     \@ifnotempty{##2}{\ifnum\cdr@thankcount=\z@\else, \fi\href{mailto:##2}{##2}\@ifnotempty{##1}{ \mbox{(##1)}}}\endgroup\fi
     \global\advance\cdr@thankcount\@ne}%
   \def\urladdr##1##2{\relax}%
   \sbox\@tempboxa{\addresses\xdef\CDRess{\ifnum\cdr@thankcount>\@ne\relax s\fi}}%
   \ifdim\wd\@tempboxa>1em\relax
   \vskip2pt\@@par\textit{\emailsaddrname{}\CDRess\thsp:} 
   \cdr@thankcount\z@
   \addresses%\@addpunct.%
   \fi
   \endgroup
 }
\def\@setcurraddr{%\par
  \begingroup
   \cdr@thankcount\z@
   \ifcdr@hyperref  \url@samestyle
   \else\def\url##1{##1}%
   \def\href##1##2{##2}\fi
   \def\affiliationonly##1{\relax}%
   \def\snailmailonly##1{\relax}%
   \def\lastname##1{\relax}%
   \def\firstname##1{\relax}%
   \def\hasthanks##1{\relax}
   \def\hasaddress##1{\relax}%
   \def\author##1{}%\ifnum\cdr@thankcount=\z@\else, \fi}
   \def\address##1##2{\relax}%
   \def\doauthorinfo##1{\relax}%
   \def\curraddr##1##2{%% Showing current addresses?
     \ifcdr@GroupEmails
     \begingroup
     \@ifnotempty{##2}{\ifnum\cdr@thankcount=\z@\else, \fi##2\@ifnotempty{##1}{ \mbox{(##1)}}}\endgroup\fi
     \global\advance\cdr@thankcount\@ne}%
   \def\email##1##2{\relax}%
   \def\urladdr##1##2{\relax}%
   \sbox\@tempboxa{\addresses\xdef\CDREss{\ifnum\cdr@thankcount>\@ne\relax es\fi}}%
   \ifdim\wd\@tempboxa>1em\relax
   \vskip2pt\@@par\textit{\curraddrname{}\CDREss\thsp:} 
   \cdr@thankcount\z@
   \addresses%\@addpunct.%
   \fi
   \endgroup
 }
%%%% Fin pres aut

%% Footnotes 1st page
\def\@adminfootnotes{}%
%   \let\@makefnmark\relax  \let\@thefnmark\relax
%   \begingroup\normalparindent0pt\footnotesep10pt\relax
%\endgroup}
\def\@setsubjclass{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\subjclassname.}\kern.25em\ignorespaces
  \@subjclass\@addpunct{{\upshape.}}\par}
\RequirePackage[french,english,iso]{isodate} % TODO treat that with language selection
\origdate
\RequirePackage[shortlabels]{enumitem}  
\setlist{font=\upshape}
\newif\ifcdr@revisedaccepted\cdr@revisedacceptedfalse
\newif\ifcdr@receivedaccepted\cdr@receivedacceptedfalse
\def\datererevised#1{\def\@datererevised{#1}}%
\let\@datererevised\@empty
\def\daterevisedaccepted#1{\def\@daterevised{#1}\def\@dateaccepted{#1}\cdr@revisedacceptedtrue}
%
 \def\@setdate{%
   \ifx\@empty\@dateaccepted \MissingInfo{This article is a draft (not yet accepted!)}%
   \else 
  \if@francais
    \itshape\selectlanguage{french}%
    \noindent Manuscrit \ifx\@empty\cdr@presentedby\else pr\'esent\'e
    par \cdr@presentedby, \fi re\c cu  
      \ifcdr@receivedaccepted et accept\'e le \printdate\@datereceived
      \else
        le \printdate\@datereceived,
        \ifcdr@revisedaccepted	
           r\'evis\'e et  accept\'e le \printdate\@dateaccepted
        \else
          \ifx\@empty\@daterevised
          \else
            r\'evis\'e le \printdate\@daterevised
              \ifx\@empty\@datererevised
              \else\ et le \printdate\@datererevised
              \fi, 
          \fi
          accept\'e le \printdate\@dateaccepted
        \fi
      \fi.
  \else
    \itshape\selectlanguage{english}%
    \noindent Manuscript \ifx\@empty\cdr@presentedby\else presented
    by \cdr@presentedby, \fi received
    \ifcdr@receivedaccepted and accepted \printdate\@datereceived
    \else
     \printdate\@datereceived,
     \ifcdr@revisedaccepted
      revised and  accepted  \printdate\@dateaccepted
     \else
      \ifx\@empty\@daterevised
      \else
        revised  \printdate\@daterevised
        \ifx\@empty\@datererevised
        \else\ and
         \printdate\@datererevised
        \fi,
      \fi
       accepted  \printdate\@dateaccepted
     \fi
     \fi.
   \fi
\fi}
\ifcdr@Thematic
    \AtBeginDocument{%
        \let\@datereceived\@empty
        \let\@daterevised\@empty
        \let\@dateaccepted\@empty
        \let\@datererevised\@empty
    }%
    \def\@setdate{
        \ifx\@dateposted\@empty\else 
            \ifcdr@efirst Online first, \else Available online \fi
            {\selectlanguage{english}\printdate{\@dateposted}}
        \par\fi
    }
\fi
%
\def\dedicatoryfont{\normalfont\footnotesize\itshape}
\def\@setdedicatory{%
    \begingroup
      \def\signature##1{\nobreak\hskip 2em plus 1fil
        \penalty-5\hbox{}\nobreak\hfil\parfillskip=0pt
        \mbox{\upshape ##1}\par}
      \raggedleft
      \dedicatoryfont
      \@dedicatory\par
    \endgroup}
\def\@setkeywords{%
  \global\kwd@count=\z@%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\keywordsname.}\kern.25em\ignorespaces
  \@keywords\unskip\@addpunct{{\upshape.}}\par}
\def\@setaltkeywords{%
  \global\kwd@count=\z@%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\altkeywordsname.}\kern.25em\ignorespaces
  \@altkeywords\unskip\@addpunct{{\upshape.}}\par}
\newcount\cdr@numberofthanks\cdr@numberofthanks=\z@
\def\@setthanks{\abstractfont\def\thanks##1{\ifnum\cdr@numberofthanks=\z@\relax\else\@par
   \fi##1\@addpunct{{\upshape.}}\advance\cdr@numberofthanks1\relax}{\abstractheadfont\thanksname.}\kern.25em\ignorespaces\thankses\par}
\def\@setESM{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\ESMname.}\kern.25em\ignorespaces
  \@ESM\@addpunct{{\upshape.}}\par}
\def\@settranslators{\par
  \begingroup
  \translatedby\ \andify\@translators
  {\sl \ignorespaces\@translators} \@@par
  \endgroup}
\if@francais
\def\cdr@correspondingname{Correspondance}
\def\keywordsname{Mots-cl{\'e}s}
\def\altkeywordsname{Keywords}
\def\subjclassname{Classification math{\'e}matique par sujets (2010)}
\def\thanksname{Financement}
\def\emailsaddrname{Courriel}
\def\ESMname{Mat{\'e}riel {\'e}lectronique suppl{\'e}mentaire}
\else
\def\cdr@correspondingname{Correspondance}
\def\keywordsname{Keywords}
\def\altkeywordsname{Mots-cl{\'e}s}
\def\subjclassname{Mathematical subject classification (2010)}
\def\thanksname{Funding}
\def\emailsaddrname{E-mail}
\def\ESMname{Electronic supplementary material}
\fi
\@xp\let\csname subjclassname@2010\endcsname \subjclassname
%
\def\longthankssection{\subsubsection*{Acknowledgements}}
\long\def\longthanks#1{\longthankssection

  #1}%
%
%
\def\enddoc@text{}
%
%% Page de garde
\def\@makePagedeGarde{% TODO this belongs in the main class file
\ifcdr@pagedegarde
{\makeatletter\input{CR-pagedegarde}}%
\newpage\pagecolor{white}\gdef\GPT@pageliteral{}\fi}
%
\ifcdr@sommaire
\let\cdr@postabstracthook\@empty
\def\ps@firstpage{\count@=\currentyear
  \ps@plain
  \let\@oddfoot\@empty
  \let\@evenfoot\@oddfoot
  \def\@oddhead{\@serieslogo\hss}%
  \let\@evenhead\@oddhead % in case an article starts on a left-hand page
}
%
\let\ps@headings\ps@empty
\let\ps@plain\ps@empty
\def\article@logo{%
    \set@logo{%
        \hsize\textwidth
        {\Large\textit{Comptes Rendus\\\CDRcrasseries}\\[2pt]}%
        \ifx\@empty\currentvolume
            \textbf{Draft}
        \else
            \textbf{\currentyear},
            \currentvolume
            \ifx\currentissue\@empty\else, \no\currentissue
        \fi\fi\\
        \mbox{}%
        \hfill
        \raisebox{-3mm}[0pt][0pt]{\includegraphics[height=16mm]{Logo_Academie_grisfonce.pdf}}\\[18bp]
        \centerline{\rule{.8\textwidth}{1.5bp}}
    }%
}
%
\def\smfbyname{\vspace*{-17mm}}
\def\lastname#1{#1}
\def\junior#1{\unskip, #1}%
\renewcommand{\@pnumwidth}{4.5em}
\def\@adminfootnotes{}
\def\enddoc@text{}
%% 
\fi
\ifcdr@volume
    \def\@makefront{%
        \IncludeSom{\cdr@journal -Sommaire}%
        \cleardoublepage
        \ifcdr@SOM
            \@makeSOM
            \begingroup\makeatletter
                \newcommand\SomLine[9]{%
                    \gdef\cdr@shortresps{##1}%
                    \gdef\cdr@resps{##2}%
                    \gdef\cdr@specialtitle@french{##5}%
                    \gdef\cdr@specialtitle@english{##4}%
                    \gdef\cdr@specialabstract@french{##7}%
                    \gdef\cdr@specialabstract@english{##6}%
                }%
                \InputIfFileExists{./\CDRidvol.cdrsom}{%
                    \message{** Fichier  \CDRidvol.cdrsom charge  **^^J}}{%
                    \message{** Pas de fichier \CDRidvol.cdrsom  pour ce volume !**^^J}}%
            \makeatother\endgroup
        \fi
    }
    \def\@makebody{%
        \ifcdr@newsom\ShellEscape{rm -f \cdr@journal-Sommaire-data.tex}\fi
        % \ifcdr@specialtitre
        %   \newwrite\cdr@globalcfgfile
        %   \immediate\openout\cdr@globalcfgfile=\CDRidvol -global.cfg
        %   \immediate\write\cdr@globalcfgfile{\the\cdr@specialtitret}%
        %   \immediate\closeout\cdr@globalcfgfile
        % \fi
        \pagenumbering{arabic}%
        \setcounter{page}{\@FirstPage}%
        \tkkp={\setpage}%
    }
    \def\enddoc@text{}
\else
    \ifcdr@sommaire %% Sommaire
        \AtEndOfClass{%
            \begingroup\makeatletter
                \newcommand\SomLine[9]{%
                    \gdef\cdr@shortresps{#1}%
                    \gdef\cdr@resps{#2}%
                    \gdef\cdr@specialtitle@french{#5}%
                    \gdef\cdr@specialtitle@english{#4}%
                    \gdef\cdr@specialabstract@french{#7}%
                    \gdef\cdr@specialabstract@english{#6}%
                }
                \InputIfFileExists{./\CDRidvol.cdrsom}{%
                    \message{** Fichier  \CDRidvol.cdrsom charge  **^^J}%
                    %  \let\SomLine\undefined
                    }%
                    {\message{** Pas de fichier \CDRidvol.cdrsom  pour ce volume !**^^J}}%
            \makeatother\endgroup
        }
        \AtBeginDocument{%
            \newcommand\SomLine[9]{%
                \def\lng{#3}%
                \def\LNG{french}%
                \par \addpenalty\@secpenalty\addvspace{\medskipamount}%
                \begingroup
                    \hyphenpenalty50\def\\{\allowbreak}%
                    \parindent0pt
                    %    \parindent-\normalparindent \leftskip\normalparindent\relax 
                    \rightskip\@pnumwidth% plus6em
                    {\bfseries\ignorespaces#2\unskip}\@par
                    \parfillskip-\@pnumwidth
                    %    \hskip1em
                    \href{\CDRidvol.pdf\#page.#8}{\ifx\lng\LNG#5\else#4\fi}\unskip\leavevmode
                    % TODO use named destination instead of page number
                    \nobreak\hskip2pt\nobreak \leaders\hbox{$\m@th \mkern 1.5mu\hbox{.}\mkern 1.5mu$}\hfill \nobreak
                    \hb@xt@\@pnumwidth{\@tocpagenum{\ignorespaces#8\unskip-\ignorespaces#9\unskip}}%
                    \par
                \endgroup
                %    \begingroup\parindent\normalparindent\relax\leftskip2.4em\footnotesize\ignorespaces#7\unskip\par
                %    \endgroup
            }
        }
    \else %% Articles
        \AtEndOfClass{%
            \begingroup\makeatletter
                \newcommand\SomLine[9]{%
                    \gdef\cdr@shortresps{#1}%
                    \gdef\cdr@resps{#2}%
                    \gdef\cdr@specialtitle@french{#5}%
                    \gdef\cdr@specialtitle@english{#4}%
                    \gdef\cdr@specialabstract@french{#7}%
                    \gdef\cdr@specialabstract@english{#6}%
                }%
                \InputIfFileExists{../\CDRidvol.cdrsom}{%
                    \message{** Fichier  \CDRidvol.cdrsom charge pour cet article **^^J}}{%
                    \message{** Pas de fichier \CDRidvol.cdrsom  pour ce volume !**^^J}}%
            \makeatother\endgroup
        }
    \fi
\fi

%AJOUTS CS
%\RequirePackage{amssymb,upref}

\NumberTheoremsIn{}
\setcounter{tocdepth}{3}

%% Thms
\ifcdr@ThmDefs\OneNumberAllTheorems\fi
\def\th@plain{%
  \thm@bodyfont{\normalfont\itshape}%
  \thm@headfont{\normalfont\bfseries}%
  \thm@notefont{\normalfont\bfseries}%
  \thm@headpunct{.\kern.2em\ignorespaces}%
  \let\thm@indent\noindent 
  \def\thm@space@setup{%
    \thm@preskip=\smallskipamount
    \thm@postskip=\thm@preskip}%
  \itshape
}
\def\th@remark{%
  \thm@bodyfont{\normalfont}%
  \thm@headfont{\normalfont\bfseries}%
  \thm@notefont{\normalfont\bfseries}%
  \thm@headpunct{.\kern.2em}%
  \let\thm@indent\noindent 
  \def\thm@space@setup{%
    \thm@preskip=\smallskipamount
    \thm@postskip=\thm@preskip}%
}
\let\th@definition\th@plain
%\def\cdr@proofindent{\z@}%{1.5\parindent}
\renewenvironment{proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\cdr@proofindent
        {\providecommand\printref{\relax}%
\bfseries
    #1\@addpunct{\cdr@proofpunct}}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
%% Sectionning 
\def\@startsection#1#2#3#4#5#6{%
 \if@noskipsec \leavevmode \fi
 \par \@tempskipa #4\relax
 \@afterindenttrue
 \ifdim \@tempskipa <\z@ \@tempskipa -\@tempskipa \@afterindentfalse\fi
 \if@nobreak \everypar{}\else
     \addpenalty\@secpenalty\addvspace\@tempskipa\fi
 \@ifstar{\@dblarg{\@sect{#1}{\@m}{#3}{#4}{#5}{#6}}}%
         {\@dblarg{\@sect{#1}{#2}{#3}{#4}{#5}{#6}}}%
}
\def\@seccntformat#1{%
  \protect\textup{\protect\@secnumfont
    \csname the#1\endcsname
    \protect\@secnumpunct
  }%
}
\def\@sectionfamily{\normalfont}
\def\@sectionfont{\@sectionfamily\large\bfseries}
\let\contentsnamefont\@sectionfont
\def\@secnumfont{\selectfont}
%\def\@upn{\normalfont\selectfont}
\def\@subsectionfont{\@sectionfamily\large\itshape}
\def\@subsubsectionfont{\@sectionfamily\itshape}
\def\@paragraphfont{\normalfont\bfseries}


\def\section{\@startsection{section}{1}%
  \z@{-1.5\linespacing\@plus-.5\linespacing\@minus-.5\linespacing}{.8\linespacing\@plus.2\linespacing\@minus.3\linespacing}%
  {\@sectionfont}}
\def\subsection{\@startsection{subsection}{2}%
  \z@{-1.5\linespacing\@plus-.5\linespacing\@minus-.5\linespacing}{.8\linespacing\@plus.2\linespacing\@minus.3\linespacing}%
  {\normalfont\@subsectionfont}}
\def\subsubsection{\@startsection{subsubsection}{3}%
  \z@{.5\linespacing\@plus.5\linespacing}{.5\linespacing}%
  {\normalfont\@subsubsectionfont}}
\def\paragraph{\@startsection{paragraph}{4}%
  \z@{.5\linespacing\@plus.5\linespacing}{-\fontdimen2\font}%
  {\normalfont\@paragraphfont}}
%
\newcount\tochyphenpenalty
\tochyphenpenalty\@M
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\tochyphenpenalty
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax
      \advance\leftskip\@tempdima\relax
    \advance\rightskip\@pnumwidth % plus1em
    \parfillskip-\@pnumwidth
    {#5{\leavevmode\hskip-\@tempdima #6}}%
    \nobreak
    \xleaders\hbox to1ex{\normalfont\hss.\hss}\hfil\nobreak
    \hbox to\@pnumwidth{\@tocpagenum{#7}}\par
    \nobreak
    \endgroup
  \fi}
%
\renewcommand{\tocpart}[3]{%
  \indentlabel{\@ifnotempty{#2}{\ignorespaces#1 #2.\kern1ex}}#3}
\let\tocsection\tocpart
\let\tocsubsection\tocsection
\let\tocsubsubsection\tocsection
\let\tocparagraph\tocsection
\def\l@part{\@tocline{-1}{12pt plus2pt}{0pt}{}{\bfseries\smf@boldmath}}
\def\l@section{\@tocline{1}{0pt}{0pc}{}{}}
\def\l@subsection{\@tocline{2}{0pt}{1pc}{}{}}
\def\l@subsubsection{\@tocline{3}{0pt}{2pc}{}{}}
\def\l@paragraph{\@tocline{5}{0pt}{3pc}{}{}}
\def\l@figure{\@tocline{0}{3pt plus2pt}{0pt}{}{}}
\let\l@table\l@figure
%
\def\@smfprotect{\let\smfcr\\\def\\{\protect\smfcr}}
\DeclareRobustCommand{\MakeUppercase}[1]{{%
    \@smfprotect\upchars@
    \protected@edef\reserved@a{#1}\uppercasenonmath\reserved@a\reserved@a}}
\protected@edef\MakeUppercase#1{\MakeUppercase{#1}}
%
% \def\@makefnmark{%
%   \leavevmode
%   \raise.9ex\hbox{\fontsize\sf@size\z@\normalfont(\@thefnmark)}%
% }%CS
%
%% Additional macros %%
\AtBeginDocument{%
    \csname url@samestyle\endcsname
    \begingroup
        \ifx\@dateposted\@empty
            \ifnum\currentvolume=\z@%
                \def\setpdftimes#1#2{\gdef\@dateposted{#2}}%
                \ifcdr@published
                    \InputIfFileExists{\jobname-pdftimestamp.txt}{}{}% TODO this is repeating something from cedram.cls
                \else
                    \cdr@mkfile{\jobname-pdftimestamp.txt}{\string\setpdftimes{\pdftex@now}{\@dateprod}}
                    \edef\cdr@tmp@{\pdftex@now}
                    \expandafter\setpdftimes\expandafter{\cdr@tmp@}{\@dateprod}%
                \fi
                \cdr@mkfile{\jobname-dateposted.txt}{\string\dateposted{\@dateposted}}%
            \else
                \InputIfFileExists{\jobname -dateposted.txt}{}{}% TODO job-dateposted.txt files are obsolete if \dateposted is from PTF
            \fi
        \fi
    \endgroup
}
\emergencystretch2em
\arraycolsep 1.5pt
%%
\def\etal{{\normalfont\itshape et al.}}

\def\sautpage{\vadjust{\pagebreak}}
\newcommand\PB{\pagebreak}
\newcommand\SP{\sautpage}
\newcommand\SPB{\sautpage\break}
\newcommand\PBI{\pagebreak\noindent}


\endinput


%% predefined macros
\let\le\leqslant
\let\ge\geqslant 
\let\leq\leqslant   
\let\geq\geqslant
\let\emptyset\varnothing
\def\sfrac#1#2{{#1}/{#2}}
\def\loccit{loc.\kern3pt cit.\kern.3em}
\def\cf{cf.\kern.3em}
\def\eg{e.g.\kern.3em}
\def\ie{i.e.\kern.3em}
\def\resp{\text{resp.}\kern.3em}
\def\etc{etc.\kern.3em}
\let\ecc\etc
\let\oldsetminus\setminus
\let\setminus\smallsetminus
\newcommand{\arXiv}[1]{\href{http://arxiv.org/abs/#1}{\texttt{arXiv\string:\allowbreak#1}}}
\newcommand{\eprintHal}[1]{\href{https://hal.archives-ouvertes.fr/hal-#1}{\texttt{hal-#1}}}

\AtEndOfClass{%
\let\oldbigoplus\bigoplus
\let\oldbigcup\bigcup
\let\oldbigcap\bigcap
\let\oldbigotimes\bigotimes
\let\oldbigwedge\bigwedge
\let\oldcoprod\coprod
\def\sautpage{\vadjust{\pagebreak}}
\newcommand\PB{\pagebreak}
\newcommand\SP{\sautpage}
\newcommand\SPB{\sautpage\break}
\newcommand\PBI{\pagebreak\noindent}
}
\AtBeginDocument{%
\url@samestyle
\def\bigoplus{\mathop{\textstyle\oldbigoplus}\displaylimits}%
\def\bigcup{\mathop{\textstyle\oldbigcup}\displaylimits}%
\def\bigcap{\mathop{\textstyle\oldbigcap}\displaylimits}%
\def\bigotimes{\mathop{\textstyle\oldbigotimes}\displaylimits}%
\def\bigwedge{\mathop{\textstyle\oldbigwedge}\displaylimits}%
\def\coprod{\mathop{\textstyle\oldcoprod}\displaylimits}%
}

